Columnar Formats for Schemaless LSM-based Document Stores

In the last decade, document store database systems have gained more traction for storing and querying large volumes of semi-structured data. However, the flexibility of the document stores' data models has limited their ability to store data in a columnar-major layout - making them less performant for analytical workloads than column store relational databases. In this paper, we propose several techniques based on piggy-backing on Log-Structured Merge (LSM) tree events and tailored to document stores to store document data in a columnar layout. We first extend the Dremel format, a popular on-disk columnar format for semi-structured data, to comply with document stores' flexible data model. We then introduce two columnar layouts for organizing and storing data in LSM-based storage. We also highlight the potential of using query compilation techniques for document stores, where values' types are known only at runtime. We have implemented and evaluated our techniques to measure their impact on storage, data ingestion, and query performance in Apache AsterixDB. Our experiments show significant performance gains, improving the query execution time by orders of magnitude while minimally impacting ingestion performance.

==> __latexindent_temp.tex <==
\begin{figure*}[t]
%    \centering
    \begin{subfigure}[b]{0.42\textwidth}
        \includegraphics[width=\textwidth, height=0.56\textwidth]{figures/dremel_1.pdf}
        \caption{}
        \label{fig:schema-struct-1}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth, height=0.5\textwidth]{figures/dremel_2.pdf}
        \caption{}
        \label{fig:schema-struct-2}
    \end{subfigure}
    \caption{\textbf{(a)} An ADM record \textbf{(b)} Inferred schema tree structure \textbf{(c)} Dictionary-encoded field names}
    \label{fig:schmea-strcut}
\end{figure*}
\section{Flexible Columnar Format for nested semi-structured data}
\label{dremel}
One of the main reasons that document stores are not supporting storing the data in a columnar format is the flexibility of their data model. Dremel (or Parquet) format requires a schema that describes all fields to be declared a priori, where all fields must conform to one type. In this section, we give a brief overview of the Dremel format. Then, we present our extensions to Dremel to allow schema changes, such as adding new values and changing their types.

\subsection{Dremel Format}
Dremel format allows for storing nested records in a columnar fashion, where atomic values of different records are stored contiguously. For better illustration, Figure x shows an example of three JSON records about video gamers stored in Dremel format along with the user-declared schema. The schema's inner nodes resemble the nested values (objects and arrays), whereas the leaf nodes represent the atomic values such as integers and strings. The schema describes the JSON records structure, where the root has three fields id, name, and games of types of integer, object, and array, respectively. The name object consists of first and last name pairs, both of which are of type string. Next is the array of objects games, which stores information about the gamers' owned games, namely the games' titles and the different versions of a game the gamers own for different consoles. Every value (nested or atomic) in our example is optional except for the record's key id. The optionality of all non-key values is synonymous with the schema-less document stores model, which is the scope of this paper. We encourage interested readers to refer to \cite{dremel, dremel-made-simple} for more details on the representation of non-optional values.
 
 The tables below the leaf nodes shown in Figure x illustrate Dremel's columnar-striped representation of the records' atomic values shown in Figure x. Each table consists of three columns: R, D, and Value, where R and D denote the Repetition-Level and Definition-Level of each Value as presented in [x]. The repetition and definition level's roles determine the start and end of a repeated value (array) and the NULL occurrence level for a nested value, respectively. The pairs (R:x, D:y), shown at the top of each table in Figure x, indicate the maximum value for the repetition and definition levels for each atomic value.
 
To illustrate, the column $name.first$ has a maximum repetition level set to 0, which indicates a non-repeated value (or not an array's element), whereas the definition level set to 2, which is the level of the leaf node in the schema's tree ($root$ (0) $\rightarrow$ $name$ (1) $\rightarrow$ $first$ (2)). In the first record \textcircled{1} in Figure x, the definition level for the value $name.first$ is 0, which indicates that only the root was present in the path (root $\rightarrow$ first). Thus, the value for the $name.first$ in the first record in our example is NULL. For the second record \textcircled{2}, the definition level for the same value is 1, which indicates the name object is present but not the atomic value $first$. In record \textcircled{3}, the gamer's first name is "John"; hence, the definition level is 2. In the last record \textcircled{4}, the first name value is missing, indicated by the definition level 0. In contrast to the $name.first$ column, the key field id is required for all records and the key's definition level value is ignored. Thus, the id's maximum definition level is 0.
 
 For repeated values (array elements) such as the games' titles column (denoted as $games[*].title$) in our example, the repetition levels determine the array starts and ends for each record. Note that for the repeated values $games[*].title$, the maximum repetition and definition levels are 1 and 3, respectively. For example, the first record has only one value (0, 3, "NFL"), where the triplet (r, d, v) denotes the repetition level (r), definition level (d), and value (v), respectively. The repetition level 0 indicates that the value "NFL" is the record's first $games[*].title$ repeated value, and the definition level 3 indicates that the value is present. The following value (0, 3, "FIFA) corresponds to the second record as the repetition level 0 indicates the current value is, again, the first $games[*].title$ repeated value for the second record. Similarly, the value (0, 3, "NBA") corresponds to the third record; however, the following value (1, 3, "NFL") also corresponds to the same record (i.e., the second element of the array), which is indicated by repetition level 1. Therefore, whenever a value's repetition level is equal to the column's maximum repetition level, we know that it is the $i^{th}$ repeated value (or $i^{th}$ element of the array), where $i > 0$. In the last record, the array $games$ itself is missing, and thus its definition level is 0.
 
 In Figure x, the array "consoles" (the full path denoted as $games[*].consoles[*]$) is an ancestor of the outer array $games$. Therefore, the maximum repetition level for the column $games[*].consoles[*]$ is 2, as shown in Figure x. Like in the column $games[*].title$, the value (0, 2, NULL) corresponds to the first record, as indicated by the repetition level 0. However, the first record is missing the field consoles; thus, the definition level 2 indicates that the consoles array is missing but not its object parent. The following value (0, 4, "PC") is the first $games[*].consoles[*]$'s value for the second record as indicated by its repetition level 0. The definition level 4 here means that the value is present (or not NULL) and the value is "PC". The next value (2, 4, "PS4") has a repetition level 2, the maximum repetition level for the column $games[*].consoles[*]$, which means it is the second value of the array consoles. Likewise, the following two values (0, 4, "PS4") and (2, 4, "PC") correspond to the last record, and both constitute the first and second elements of the first consoles array. The following value's (1, 4, "XBOX") repetition level 1 means it still corresponds to the same record; however, the value marks the beginning of the second consoles' array, which has a single element "XBOX". The last value (0, 0, NULL) indicates (again) the array $games$ is missing from the last record.
 
 \subsection{Extended Dremel Format}
 
Dremel format, as summarized earlier, is designed for storing semi-structured data such as JSON documents in a columnar-oriented fashion. However, the requirement of declaring the schema a priori prohibits document stores from adopting it. Additionally, the Dremel format does not support union types, where a value (or a column) can be of different types in different records. In this section, we present our extensions to the Dremel format for LSM-based document stores to accommodate their flexible data model. 


\subsubsection{\textbf{Array Values:}}
Earlier, we showed the Dremel approach for representing repeated values (arrays) using the repetition levels. We observe that the repetition levels (i) are redundant among nodes that share the same ancestor array, and (ii) along with the definition levels, they occupy more bits than needed to represent optional repeated values. 

In our example shown in Figure x, we notice that the repetition levels of the column $games[*].name$ is a subset of the column $games[*].consoles[*]$'s repetition levels (redundancy), as both share the same array ancestor $games[*]$. Namely, the entire repetition levels of the column $games[*].title$  [0, 0, 0, 1, 0] appear in the same order as in the column $games[*].consoles[*]$'s repetition levels [\textbf{0}, \textbf{0}, 2, \textbf{0}, 2, \textbf{1}, \textbf{0}]. For (ii), we observe that all values with repetition levels greater than 0 must have definition levels greater or equal to the array's level. Recall that a value with repetition levels greater than 0 corresponds to the $i^{th}$ element of an array, where $i > 0$. When the repetition level is greater than 1, it implies an array exists, and its length is greater than one. Also recall that when the definition level is smaller than an array's level in the schema, it means the array itself is NULL. Therefore, having a repetition level greater than 0 and a definition level smaller than the array's level is contradictory. In other words, it means the array exists, and its length is greater than one, but the array itself is NULL (or does not exist). Given that, the number of bits of both the definition and repetition levels is more than we need to represent repeated values. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.39\textwidth]{figures/delimited_array.pdf}
    \caption{After deleting the record shown in Figure~\protect\ref{fig:schema-struct-1}}
    \label{fig:schema_after_delete}
\end{figure}

For the two reasons explained earlier, we opted for a different approach to represent repeated values. Recall (ii), which says the i$^{th}$ definition level (where $i>0$) of a repeated value cannot be smaller than the array's definition level. Thus, we use such definition level values as delimiters. To illustrate, Figure x shows the values of both $games[*].title$ and $games[*].conosoles[*]$ columns for the records in Figure x using the proposed approach. In the proposed approach, the repeated values in both columns have the same definition levels as in the original Dremel format. However, the definition levels could also indicate the end-of-array by having a delimiter value. In the column $games[*].title$, the first three records' repeated values are delimited by the definition level 0, which is the \textit{max-delimiter} value in the column as shown in Figure x. The value that follows a delimiter indicates the start of the next array, and the value itself is the array's first value - except for the last repeated value, where the definition level 0 indicates the array $games$ is NULL in the last record. Note that the last value's definition level 0 cannot be a delimiter since it is the first value after the preceding delimiter.

In the case of nested arrays, as in the column $games[*].consoles[*]$, the max-delimiter is 1, which indicates that the two delimiter values 0 and 1 are for the outer ($games$) and inner ($consoles$) arrays, respectively. The first value in the column $games[*].consoles[*]$ is NULL with definition level 2, which indicates the outer array $games$ is present but its element is NULL. The following value is a delimiter of the outer array $games$ indicated by the definition level 0. The next two values are the first and second array elements of the second record's array $consoles$, followed by a delimiter with the definition level 0. We omit the definition level 1, the delimiter for the inner array consoles, since the delimiter 0 encompasses the inner delimiter 1. The following two values are the first and second elements of the first $consoles$ array in the third record. The next delimiter 1 here indicates the end of the first consoles array, and the next value marks the start of the second $consoles$ array in the same record. The following delimiter 0 indicates the end of repeated values in the third record. In the last value, the definition level 0 implies the $games$ array is NULL in the last record. Like the last value of the column $games[*].title$, the definition level 0 here is not a delimiter as it is the first value after the last delimiter.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.44\textwidth, height=0.16\textwidth]{figures/popouts_3.pdf}
%    \caption{After deleting the record shown in Figure~\protect\ref{fig:schema-struct-1}}
%    \label{fig:schema_after_delete}
%\end{figure}

%\subsubsection{\textbf{Handling Dynamic Schemas}}
%For LSM-based document stores, one could use the approach proposed in [x] (and summarized in Section x) to obtain the schema by performing a single pass into the flushed records and then dissecting the flushed records into columns in a second pass. The two-pass approach is feasible as the flushed records reside entirely in memory (although a single-pass is sufficient in our extension, as we explain later). However, after the initial flush, the subsequent flushes could infer new columns the previously dissected records did not have and, consequently, they must reflect those changes. Let us assume that the memory budget can accommodate only a single record, and the first record (with id = 0) is flushed first to disk. Figure x shows the sequence of changes in the object name's schema in each flush, where in the first flush, the object name is missing. After flushing the second record (with id = 1), we infer the new column $name.first$. Consequently, we need to set the newly inferred column's definition level to 0 to the previously flushed record, as expected in the Dremel format and shown in Figure x. Similarly, we need to set the definition levels of the newly inferred column $name.first$ to 0 and 1, for the records with ids equals to 0 and 1, respectively, after the third flush. Adding the definition and repetition levels of newly inferred columns for all previously flushed records is not practical, as new columns could appear after inserting millions of records or even possible due to the LSM immutability. 
%
%In document stores, a value is always accessed by specifying the path from the root to the desired value (whether it is nested or atomic). When the schema is missing part (or all) of the desired path, the resulting value is always NULL. For example, accessing the value of the column $name.first$ in the first record using the schema obtained from the first flush in Figure x produces NULL, as the object name is missing. Similarly, accessing the same value in the second record using the second flush schema will always produce NULL, as the field last is missing from the object name; however, the result of accessing the column $name.last$ produces the value "Brown". Observe that the existence of an atomic value in a record always implies the parents' existence. Using this notion, the existence of the value $name.last$ in the second record implies the definition level for the missing sibling column $name.first$ is 1. Note that the result of accessing a missing column (e.g., $name.first$ using the second schema) is always NULL despite the sibling's ($name.last$) definition levels, and thus, we do not need to inspect the definition level of any of the siblings. When accessing the nested value $name$, all of its atomic values are stitched together to form the object $name$ using the record assembly automaton detailed in [x]. Thus, in the second record, the existence of the last name value "Brown" implies that the object $name$ exists, and the final result would be \{"last": "Brown"\}.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=0.44\textwidth, height=0.2\textwidth]{figures/popouts_2.pdf}
%    \caption{After deleting the record shown in Figure~\protect\ref{fig:schema-struct-1}}
%    \label{fig:schema_after_delete}
%\end{figure}
%



\subsubsection{\textbf{Schema Changes and Heterogeneous Values:}}

For LSM-based document stores, one could use the approach proposed in \cite{compact} (summarized in Section x) to obtain the schema and use it to dissect the values into columns. However, one primary challenge for supporting columnar formats in document stores is handling heterogeneous values. For example, the two records \lstinline[language=AQLSchema,basicstyle=\noindent\small]|{"id": 1, "age": 25}| and \lstinline[language=AQLSchema,basicstyle=\noindent\small]|{"id": 2, "age": "old"}| are valid records and both could be stored in a document store. Similarly, document stores allow storing an array within a record that consists of heterogeneous values such as the array \lstinline[language=AQLSchema,basicstyle=\noindent\small]|[0, "1", {"seq": 2}]|. Limiting the support of storing the data in a columnar format to datasets with homogeneous values is probably enough for most cases, as evidently shown by the popularity of Parquet. However, including the support for datasets with heterogeneous values is a desired feature for certain use cases, especially when the users have no control over how the data is structured, like ingesting data from web APIs \cite{schema-change1, schema-change2}. In this section, we detail our approach for handling schema changes and heterogeneous types.

In our previous work \cite{compact}, we introduced union types in our inferred schemas to represent values with heterogeneous types. Figure x depicts an example of two records with their inferred schema. The inferred schema shows that the records have different types for the same value. First is the field $name$, which could be a string or an object. Thus, we infer that the $name$'s type is a union of string and object. The second union type corresponds to the $games$ array's elements, where each element could be of type string or array of strings. In the schema, we observe that union nodes resemble a special case of $object$ nodes, where the keys of the union nodes' children are their types. For example, the union node of the field $name$, in the schema shown in Figure x, has two children, where the key "object" corresponds to the left child, and the key "string" corresponds to the right child. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth, height=0.16\textwidth]{figures/union_1.pdf}
    \caption{After deleting the record shown in Figure~\protect\ref{fig:schema-struct-1}}
    \label{fig:schema_after_delete}
\end{figure}

\begin{figure}[ht]
    \includegraphics[width=0.40\textwidth, height=0.2\textwidth]{figures/union_2.pdf}
    \caption{After deleting the record shown in Figure~\protect\ref{fig:schema-struct-1}}
    \label{fig:schema_after_delete}
\end{figure}

We can dissect the unions' atomic values by treating them as object atomic values with a single modification. Observe that in a record, a value can only be of a single type. Hence, only a single value can be present, and the other atomic values of a union should be NULLs, whereas, in the atomic values of an object, all or some of the values can be present. To better illustrate, we run an example where the records are inserted one after the other, and the schema changes accordingly. Dissecting the records' values into columns is performed while inferring the schema in a single pass as in the compaction process in \cite{compact}. After inserting the first record in Figure x, we infer field $name$ is of type string, and thus we write the string value "John" with definition level 1 as shown in column \bluecircle{1} in Figure x. In the following record, the field $name$ is an object consisting of $first$ and $last$ fields. Therefore, we change the field $name$'s type from string to a union type of string and object as shown in Figure x. As the second record is the first to introduce the field $name$ as an object, we write NULLs in the newly inferred columns \redcircle{2} and \redcircle{3} for all previous records. Then, we write the values "Ann" and "Brown" with definition levels 2 in \redcircle{2} and \redcircle{3}, respectively. Recall that only a single value can be present in a union type; therefore, we write a NULL in column \bluecircle{1}. After injecting the union node in the path root $\rightarrow$ union $\rightarrow$ string, we do not change the definition level of column \bluecircle{1} from 1 to 2 for two reasons. First, union nodes are logical guides and do not appear physically in the actual records. Therefore, we ignore the union node as being part of the paths when setting the definition levels even for the two newly inferred columns \redcircle{2} and \redcircle{3}. The second reason is more technical --- changing the definition levels for all previous records is not practical, as we might need to apply the change to millions of records, or even possible due to the immutable nature of LSM.

When accessing a value of a union type, we need to inspect which value is present (not NULL) by checking the values of the union type one by one. If none of the values of the union type is present, we can conclude that the requested value is NULL. In our example shown in Figure x and Figure y, accessing the $name$ goes as follows. First, we inspect the column \bluecircle{1}, which corresponds to the string child of the union. If we get a NULL from \bluecircle{1}, we need to proceed to the following type: an object with two fields, $first$ \redcircle{2} and $last$ \redcircle{3}. In this case, we need to inspect one of the values' definition levels, say column \redcircle{2}. If the definition level is 0, we can conclude that the value $name$ is NULL, as the string and the object values of the union are both NULLs. However, if the definition level is 1, we know that the parent object is present, but the $first$ string value is NULL. Thus, the result of accessing the field $name$ is an object in this case. Inspecting all the values of a union type is not needed when the requested path is a child of a nested type. For instance, when a user requests the value $name.last$, processing column \redcircle{3} is sufficient to determine whether the value is present or not. Thus, the results of accessing the value $name.last$ are NULL in the first record and "Brown" in the second record.

The types of repeated values (array elements) could alternate between two or more types, as in the array $games$ in Figure x. In the first record, the elements' types of the array $games$ are either a string or an array of strings. Similar to the value $name$, when accessing the value $games$, we need to inspect both columns \bluecircle{4} and \redcircle{5} to determine which element of the two types is present. When accessing the value $games$, we see that the first value's definition level in column \bluecircle{4} is 2, which is the maximum definition of the column for the string value "NBA". Whereas in column \redcircle{5}, the definition level is 1, which indicates that the inner array of the union type is NULL. Thus, we know that the first element of the array $games$ corresponds to the string value of the union type. The following definition level 1 in column \bluecircle{4} indicates that the second element is NULL, whereas it is 3 in column \redcircle{5}, which is the maximum definition level of the column. Hence, the second element of the array is of type array of strings. As explained earlier in Section X, the array values are delimited, and thus, the two values with definition levels 3 and delimited by the definition level 1 correspond to the two elements \lstinline[language=AQLSchema,basicstyle=\noindent\small]|["FIFA", "PES"]| of the first record in Figure x. Following the delimiter, the definition level 1 in column \redcircle{5} indicates that the third element of the outer array is NULL. However, the definition level 2 in column \bluecircle{4} for the value "NFL" indicates that the third value of the outer array is a string. The delimiter 0 in both columns \bluecircle{4} and \redcircle{5} indicate the $games$'s end of values for the first record. The final result of accessing the value $games$ in the first record, therefore, is \lstinline[language=AQLSchema,basicstyle=\noindent\small]|["NBA", ["FIFA", "PES"], "NFL"]|, which preserves the original value of the record shown in Figure X. In the second record, we can see that is consists of two elements, both of which are of type string. Hence, the two NULL values in column \redcircle{5} indicate that none of the two elements are of type array of strings of the $games$'s union type.

\subsubsection{\textbf{Anti-matters:}}
In Section X, we briefly explained the process of deleting a record in an LSM-based storage engine using anti-matter entries. Anti-matter entries are special records that contain the key of the deleted record. In the example shown in Figure x, the id's maximum definition level is 0, as it is a required value. In order to represent anti-matter entries in our proposed columnar format, we set the maximum definition level for the primary key(s) values to 1, i.e., the definition levels' values could be either 0 or 1. The definition level here does not indicate whether the value is NULL or present; instead, it indicates whether the primary key value corresponds to a record or anti-matter. When the definition level of a primary key value is 0, it indicates that the primary key value is an anti-matter entry for a previously inserted record with the same key. When the definition level is 1, we know it is a newly inserted record.

\subsubsection{\textbf{Record Assembly:}}
When accessing the nested value as the nested value name in Figure x, all of its atomic values (i.e., first and last) are stitched together to form an object (e.g., \lstinline[language=AQLSchema,basicstyle=\noindent\small]|{"first": "John", "last": "Smith"}|) using the same Dremel's record assembly automaton \cite{dremel}. Also, we use the same algorithm to assemble repeated values (arrays). However, we use the delimiters to transition the state when constructing the arrays instead of the repetition levels in Dremel.


%
%\subsection{Partitioned Attributes Across (PAX)}
%PAX...
%
%\subsection{Oracle Truffle Framework}
%We use a similar approach in [x] to produce Truffle Abstract Syntax Tree (AST) for a partial part of the query plan (more details in Section xx). Each node of the AST describes a language operation such as numerical expressions (e.g., addition) and control flow statements (e.g., if-statement). Also, we specify the expected behavior (or specialization as in Truffle terminology) for each operation for the given input(s). For instance, the expected output for the logical expression 10 > "old" is NULL, where NULL is the expected output when the compared types are not compatible. After observing a few values by executing the AST in an interpreted mode, Truffle optimizes the AST and generates a bytecode to run it in the Java Virtual Machine (JVM), where the generated bytecode is optimized further into a machine code. Even though we only translate part of the plan, our evaluations show a tremendous improvement over the original execution model of AsterixDB.

